Perturbative aspects of the deconfinement transition -- Physics beyond the Faddeev-Popov model

In the case of non-abelian gauge theories, the standard Faddeev-Popov (FP) gauge-fixing procedure in the Landau gauge is known to be incomplete due to the presence of gauge-equivalent field configurations. A widespread belief is that the proper analysis of the low energy properties in this gauge requires the extension of the gauge-fixing procedure beyond the FP recipe. This manuscript reviews various applications of the Curci-Ferrari (CF) model, a phenomenological proposal for such an extension, based on the decoupling properties of Landau gauge correlators as computed on the lattice. We investigate the predictions of the model concerning the deconfinement transition of strongly interacting matter at finite temperature, first in the case of pure Yang-Mills theory and then in the case of heavy-quark Quantum Chromodynamics. We show that most qualitative aspects and also many quantitative features of the deconfinement transition can be accounted for within the CF model, with only one additional parameter, adjusted from comparison to lattice simulations. Moreover, these features emerge in a systematic and controlled perturbative expansion, as opposed to the ill-defined perturbative expansion within the FP model in the infrared. Applications at finite temperature and/or density require one to consider a background extension of the Landau gauge, the so-called Landau-deWitt gauge. The manuscript is also intended as a thorough but pedagogical introduction to these techniques, including the rationale for introducing a background, the role of the Weyl chambers, and the complications that emerge due to the sign problem in the case of a real quark chemical potential. It also investigates the fate of the correlation functions as computed in the CF model and conjectures a specific behavior for the corresponding functions evaluated on the lattice, in the case of the SU(2) gauge group.

==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Author's declaration}
\begin{SingleSpace}
\begin{quote}
\initial{I} declare that the work in this dissertation was carried out in accordance with the requirements of  the University's Regulations and Code of Practice for Research Degree Programmes and that it  has not been submitted for any other academic award. Except where indicated by specific  reference in the text, the work is the candidate's own work. Work done in collaboration with, or with the assistance of, others, is indicated as such. Any views expressed in the dissertation are those of the author.

\vspace{1.5cm}
\noindent
\hspace{-0.75cm}\textsc{SIGNED: .................................... DATE: .........................}
\end{quote}
\end{SingleSpace}
\clearpage
